Multi-agent Bayesian Learning with Adaptive Strategies: Convergence and Stability

We study learning dynamics induced by strategic agents who repeatedly play a game with an unknown payoff-relevant parameter. In each step, an information system estimates a belief distribution of the parameter based on the players' strategies and realized payoffs using Bayes' rule. Players adjust their strategies by accounting for an equilibrium strategy or a best response strategy based on the updated belief. We prove that beliefs and strategies converge to a fixed point with probability 1. We also provide conditions that guarantee local and global stability of fixed points. Any fixed point belief consistently estimates the payoff distribution given the fixed point strategy profile. However, convergence to a complete information Nash equilibrium is not always guaranteed. We provide a sufficient and necessary condition under which fixed point belief recovers the unknown parameter. We also provide a sufficient condition for convergence to complete information equilibrium even when parameter learning is incomplete.

==> belief_converge.tex <==
%%novalidate
\section{Empirical Consistency of Belief Update}

We make the following two assumptions: 

\emph{\textbf{(A1)} The probability density function $\phibar^\s(\cbar|\q)$ is continuous in $\q$ for all $\s \in \S$. }

\emph{\textbf{(A2)} 
$\theta^1(\s)>0$ for all $\s \in \S$.}

The estimated distribution of payoff given $\theta$ and $\q$ is given by: 
\begin{align*}
    \mutheta\(\c|\q\) = \sum_{\s \in \S} \theta(\s) \phi^\s(\c|\q). 
\end{align*}


\begin{definition}[Distinguishable parameters]\label{def:observe}
For any strategy profile $\q\in \Q$, parameter $s$ is distinguishable from the true parameter $\sran$ based on the realized outcome $\cbar$ if the Kullback–Leibler (KL) divergence from the distributions of $\cbar$ with $\s$ to the distribution with $\sran$ is positive, i.e.
\begin{align}\label{eq:KL_distinguishable}
    D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right) = \int_{\cbar} \phibar^{\sran}(\cbar|\q) \log\left(\frac{\phibar^{\sran}(\cbar|\q)}{\phibar^{\s}(\cbar|\q)}\right) d\cbar>0.
\end{align}
 The distinguishable parameter set with $\q$ is $\Sobserve(\q) \deleq \left\{\S|D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right)>0\right\}$. 
\end{definition}


\begin{definition}[Global identification]\label{def:global_iden}
The true parameter $\sran$ is globally identifiable if for any $\q \in \Q$, $\Sobserve(\q)=\S \setminus \{\sran\}$. 
\end{definition}

\begin{definition}[Total variation distance]
For any belief $\theta \in \Delta(\S)$ and any strategy profile $\q \in \Q$, we define the total variation distance between $\mutheta\(\c|\q\)$ and $\phi^{\sran}(\c|\q)$ as follows: 
\begin{align*}
    \delta\(\mutheta(\cdot|\q), ~\phi^{\sran}(\cdot|\q)\)= \sup_{C \in \mathcal{B}}\left\vert\mutheta(C|\q)-\phi^{\sran}(C|\q)\right\vert.
\end{align*}
% '
% Kullback–Leibler (KL) divergence from the estimated payoff distribution  to the true distribution 
% \begin{align*}
%     D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\mutheta\(\c|\q\)\right) = \int_{\cbar} \phibar^{\sran}(\cbar|\q) \log\left(\frac{\phibar^{\sran}(\cbar|\q)}{\mutheta\(\c|\q\)}\right) d\cbar,
% \end{align*}
\end{definition}

\begin{theorem}\label{theorem:belief_convergence}
Given any sequence of strategy profiles $\(\qt\)_{\t =1}^{\infty}$, under assumptions (A1) and (A2), the sequence of beliefs $\(\thetat\)_{\t=1}^{\infty}$ generated by belief update in \eqref{eq:update_belief} converges to a belief vector $\thetabar \in \Delta(\S)$ with probability 1, and 
\begin{align}\label{eq:empirical_consistent}
    \lim_{\t \to \infty}  \delta\(\muthetat(\cdot|\qt),~ \phi^{\sran}(\cdot|\qt)\)=0, \quad w.p.1.
\end{align}
Moreover, if $\sran$ is globally identifiable, then $\thetabar=\thetasran$ with probability 1, where $\thetasran(\sran)=1$ is the complete information belief vector. 
\end{theorem}

\noindent\textbf{\emph{Proof of Theorem \ref{theorem:belief_convergence}.}}\\
\emph{Part 1:} We prove that $\thetat$ converges to a belief vector $\thetabar$ with probability 1. 

First, we show that for any $\s \in \S$, $\(\frac{\theta^\t(\s)}{\theta^\t(\sran)}\)_{\t=1}^{\infty}$ is a non-negative martingale, and hence converges to a belief vector $\thetabar$ with probability 1. Note that for any $\t=1, 2, \dots $, and any parameter $\s \in \S \setminus \{\sran\}$, we have the follows from \eqref{eq:update_belief}: 
\begin{align*}
\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}= \frac{\theta^{\t}(\s) \cdot \phibar^{\s}(\ct|\qt)}{\theta^{\t}(\sran) \cdot \phibar^{\sran}(\ct|\qt)}
\end{align*}
Now, consider any initial belief $\thetazero$, any sequence of aggregate strategies $\Qhis\deleq \(\q^j\)_{j=1}^{\t-1}$ and any sequence of realized outcomes $\Costhis\deleq \(\cj\)_{\j =1}^{\t-1}$ before stage $\t$, we can compute the expected value of $\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}$ conditioned on $\thetazero$, $\Qhis$ and $\Costhis$ as follows: 
\begin{align}\label{conditional_iterate}
\mathbb{E}\left[\left.\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}\right\vert \thetazero, \Qhis, \Costhis\right]&= \frac{\thetat(\s)}{\thetat(\sran)} \cdot \mathbb{E}\left[\left. \frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)}\right\vert \thetazero, \Qhis, \Costhis \right], 
\end{align}
where $\thetat$ is updated from $\thetazero$ based on $\Qhis$ and $\Costhis$ using \eqref{eq:update_belief}, and $\qt$ is derived from $\qt$ for all $\t$. 

% Since the aggregate strategy $\qt$ depends on the past routing decisions and realized outcomes only through the updated belief $\thetat$. We can simplify \eqref{conditional_iterate} as follows: 
% \begin{align*}
% \mathbb{E}\left[\left.\frac{\theta^\t(\s)}{\theta^\t(\sran)}\right\vert \thetazero, \Qhis, \Costhis\right]&= \frac{\thetat(\s)}{\thetat(\sran)} \cdot \mathbb{E}\left[\left. \frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)}\right\vert \thetat\right]
% \end{align*}
We can check that the conditional expectation is 1: 
\begin{align*}
\mathbb{E}\left[\left. \frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)}\right\vert \thetazero, \Qhis, \Costhis \right]
=&\int_{\ct} \(\frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)} \) \cdot  \phibar^{\sran}(\ct|\qt) d \ct=1.
\end{align*}
Hence, for any $\t=1, 2, \dots$,  
\begin{align*}
\mathbb{E}\left[\left.\frac{\theta^{\t+1}(\s)}{\theta^{\t+1}(\sran)}\right\vert \thetazero, \Qhis, \Costhis\right]= \frac{\thetat(\s)}{\thetat(\sran)}, \quad \forall \s \in \S.
\end{align*}
Additionally, from \eqref{eq:update_belief}, we know that $\frac{\theta^\t(\s)}{\theta^\t(\sran)} \geq 0$. Hence, the sequence $\(\frac{\theta^\t(\s)}{\theta^\t(\sran)}\)_{\t=0}^{\infty}$ is a non-negative martingale for any $\s \in \S$. From martingale convergence theorem, we conclude that $\frac{\theta^\t(\s)}{\theta^\t(\sran)}$ converges with probability 1. 

Next, we show that the sequence $\left(\log\thetat(\sran)\right)_{\t=1}^{\infty}$ is a submartingale, and converges with probability 1. We define $\mu (\ct|\theta^{\t}, \qt)\deleq\sum_{\s \in \S} \theta^{\t}(\s)\phibar^{\s}(\ct|\qt)$. From \eqref{eq:update_belief}, we have:
\begin{align*}
    &\mathbb{E}\left[\left.\log\theta^{\t+1}(\sran)\right\vert \thetazero, \Qhis, \Costhis\right]= \mathbb{E}\left[\left.\log\(\frac{\theta^{\t}(\sran)\phibar^{\sran}(\ct|\qt)}{\muthetat(\ct|\qt)}\)\right\vert \thetazero, \Qhis, \Costhis\right]\\
    =& \log\theta^{\t}(\sran) +\mathbb{E}\left[\left.\log\(\frac{\phibar^{\sran}(\ct|\qt)}{\muthetat(\ct|\qt)}\)\right\vert \thetazero, \Qhis, \Costhis\right]\\
    =&\log\theta^{\t}(\sran) +\int_{\ct} \phibar^{\sran}(\ct|\qt) \log\(\frac{\phibar^{\sran}(\ct|\qt)}{\muthetat(\ct|\qt)}\) d \ct \\
    =& \log\theta^{\t}(\sran)+  D_{KL}\(\phibar^{\sran}(\ct|\qt)||\muthetat(\ct|\qt)\) \geq \log\theta^{\t}(\sran),
\end{align*}
where the last inequality is due to the non-negativity of KL divergence between $\phibar^{\sran}(\ct|\qt)$ and $\muthetat(\ct|\qt)$. Therefore, the sequence $\left(\log\thetat(\sran)\right)_{\t=1}^{\infty}$ is a submartingale. Additionally, since $\log\thetat(\sran)$ is bounded above by zero, by the martingale convergence theorem, $\log\thetat(\sran)$ must converge with probability 1. Hence, $\thetat(\sran)$ must also converge with probability 1.

From the convergence of $\frac{\theta^\t(\s)}{\theta^\t(\sran)}$ and $\thetat(\sran)$, we can conclude that $\thetat(\s)=\frac{\theta^\t(\s)}{\theta^\t(\sran)} \cdot \thetat(\sran)$ converges with probability 1 for any $\s \in \S$. We denote the convergent vector as $\thetabar= \(\thetabar(\s)\)_{\s \in \S}$. We can check that for any $\t$, $\thetat(\s) \geq 0$ for all $\s \in \S$ and $\sum_{\s \in \S}\thetat(\s)=1$. Hence, $\thetabar$ must also satisfy $\thetabar(\s) \geq0$ for all $\s \in \S$ and $\sum_{\s \in \S}\thetabar(\s)=1$, i.e. $\thetabar$ is a feasible belief vector. 

\vspace{0.2cm}
\noindent\emph{Part 2:} We show that $\thetabar$ satisfies \eqref{eq:empirical_consistent} with probability 1. 

For any parameter $\s \in \S \setminus \{\sran\}$, we define $\Qhats$ as the set of strategy profiles, based on which the parameter $\s$ is distinguishable from $\sran$, i.e. 
\begin{align*}
   \Qhats \deleq \left\{\Q \left\vert D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right)>0\right.\right\}.
\end{align*}
The set $\Qhats \subseteq \Q$. For any $\q \in \Q \setminus \Qhats$, we must have $D_{KL} \left(\phibar^{\sran}(\cbar|\q)||\phibar^{\s}(\cbar|\q)\right)=0$. 

Since any sequence of strategy profiles $\(\qt\)_{\t=1}^{\infty}$ is a bounded sequence, from Bolzano-Weierstrass Theorem, we know that the sequence has at least one limit point. We define the set of all limit points of the sequence $\(\qt\)_{\t=1}^{\infty}$ as $\limpq \subseteq \Q$ and $\limpq$ is non-empty. We prove \eqref{eq:empirical_consistent} for the following three cases separately: 

\vspace{0.2cm}

\noindent\emph{(Case 1:)} For any $\s \in \S \setminus \{\sran\}$, the sequence of strategies $\(\qt\)_{\t=1}^{\infty}$ does not enter the set $\Qhats$ infinitely often for any $\s \in \S$. 

In this case, we can find a finite step $\T>0$ such that for any $\t >\T$, $\qt \notin \Qhats$ for all $\s \in \S$. Then, for any $\t > \T$ and any $\s \in \S$, since $\qt \notin \Qhats$, we have $D_{KL} \left(\phibar^{\sran}(\ct|\qt)||\phibar^{\s}(\ct|\qt)\right)=0$, which implies $\phi^\s(\ct|\qt)=\phi^{\sran}(\ct|\qt)$ for all $\ct$. Then, for any $\thetat$, we have $\muthetat\(\ct| \qt\)= \sum_{\s \in \S} \thetat(\s)\phi^\s(\ct|\qt)=\phi^{\sran}(\ct|\qt)$ for all $\ct$. Hence, $D_{KL} \left(\phibar^{\sran}(\ct|\qt)||\muthetat\(\ct| \qt\)\right)=0$. Therefore, we can conclude that $\thetabar$ must satisfy \eqref{eq:empirical_consistent}.  

\noindent\emph{(Case 2:)} For any $\s \in \S$, we have $\limpq \cap \Qhats = \emptyset$.

To begin with, we argue that for any $\epsilon>0$, there exits a finite $\T>0$ such that for any $\t >\T$, $d\(\qt, \limpq\)<\epsilon$. Assume for the contrary that such finite $\T$ cannot be found, then there must exist a sub-sequence of strategy profiles $\(\qtk\)_{\k=1}^{\infty}$ such that $d\(\qtk, \limpq\)>\epsilon$ for all $\tk$. Since the infinite number of strategy profiles in the sub-sequence belong to the bounded closed set $\Q$, again from Bolzano-Weierstrass Theorem, we know that the sub-sequence must have at least one limit point, denoted as $\hat{\q}'$. Since $d\(\qtk, \limpq\)>\epsilon$ for all $\tk$, $\hat{\q}' \geq \epsilon>\frac{\epsilon}{2}$, and hence $\hat{\q}' \notin \Q'$. We then obtain a contradiction since $\Q'$ is the set of all limit points. 

In this case, for any $\q' \in \limpq$, $D_{KL} \left(\phibar^{\sran}(\cbar|\q')||\phi^\s\(\c| \q'\)\right)=0$. From assumption (A1), we know that for any $\epsilon>0$, we can find a positive number $\delta >0$ such that if $|\q-\q'|<\delta$, then  $\delta\(\phi^\s(\cdot|\qt),~ \phi^{\sran}(\cdot|\qt)\)<\epsilon$. Based on the above-mentioned argument, we know that there exists a finite step number $\T>0$ such that for all $\t>\T$, $ d\(\qt, \limpq\)<\delta$, i.e. for any $\t > \T$, $\exists \q' \in \limpq$ such that $|\qt-\q'|<\delta$. We can thus prove \eqref{eq:empirical_consistent} by concluding that for any $\epsilon>0$, there exists a $\T>0$ such that for any $\t>\T$,  $\delta\(\phi^\s(\cdot|\qt),~ \phi^{\sran}(\cdot|\qt)\)<\epsilon$. 



\noindent\emph{(Case 3:)} There exists a parameter $\s \in \S$ such that the sequence $\(\qt\)_{\t=1}^{\infty}$ enters the set $\Qhats$ infinitely often, and the joint set $\limpq \cap \Qhats \neq \emptyset$. We denote the set of such parameters as $\Sdagger$.


Our goal is to show that for any $\s \in \Sdagger$, $\thetabar(\s)=0$ with probability 1. By iteratively applying the belief update in \eqref{eq:update_belief}, we can write the belief $\thetat$ as follows: 
\begin{align}\label{eq:sequence_update}
    \thetat(\s)= \frac{\theta^1(\s) \prod_{\j=1}^{\t-1}\phibar^{s}(\cj|\q^j)}{\sum_{\s' \in \S} \theta^1(\s') \prod_{\j=1}^{\t-1}\phibar^{s'}(\cj|\q^j)}, \quad \forall \s \in \S.
\end{align}
We define $\Phi^\s(\Costhis|\Qhis)$ as the density function of the history of the realized outcomes $\Costhis$ conditioned on the history of aggregate strategies $\Qhis$ before stage $\t$, i.e. $\Phi^\s(\Costhis|\Qhis) \deleq \prod_{\j=1}^{\t-1}\phibar^{s}(\cj|\q^j)$. Then, we simplify \eqref{eq:sequence_update} as follows: 
\begin{align}
    \thetat(\s)&= \frac{\theta^1(\s) \Phi^\s(\Costhis|\Qhis)}{\sum_{\s' \in \S} \theta^1(\s') \Phi^{\s'}(\Costhis|\Qhis)} \leq \frac{\theta^1(\s) \Phi^\s(\Costhis|\Qhis)}{ \theta^1(\s) \Phi^{\s}(\Costhis|\Qhis)+ \theta^1(\sran) \Phi^{\sran}(\Costhis|\Qhis)}\notag\\
    &=\frac{\theta^1(\s) \frac{\Phi^\s(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}}{ \theta^1(\s) \frac{\Phi^{\s}(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}+ \theta^1(\sran)}\label{eq:bound_theta}
\end{align}
Hence, if we can prove that the likelihood ratio $ \frac{\Phi^\s(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}$ converges to 0 as $\t$ goes to infinity for all $\s \in \Sdagger$, then $\theta(\s)$ must also converge to 0. %To begin with, we compute the log-likelihood ratio as follows:  
% \begin{align}\label{eq:log-likelihood}
%     \lim_{\t \to \infty}\log \(\frac{\Phi^\s(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}\)=   \lim_{\t \to \infty}\sum_{\j=1}^{\t-1} \log\(\frac{\phibar^{\s}(\cj|\loadj)}{\phibar^{\sran}(\cj|\loadj)}\).
% \end{align}


Since the sequence $\(\qt\)_{\t=1}^{\infty}$ enters the set $\Qhats$ infinitely often, we have a sub-sequence of strategy profiles in the set $\Qhats$ as $\(\qtk\)_{\k=1}^{\infty}$. For any $\t \in  \{1, 2, \dots\} \setminus \{\t_1, \t_2, \dots\}$, since $\qt \notin \Qhats$, the KL-divergence $D_{KL}\(\phibar^{\sran}(\cj|\loadj)||\phibar^{\s}(\cj|\loadj)\)=0$, which implies that $\phibar^{\s}(\cj|\loadj)=\phibar^{\sran}(\cj|\loadj)$ with probability 1. Then, we can write the likelihood ratio as follows:
\begin{align}\label{eq:likelihood}
    \lim_{\t \to +\infty}\frac{\Phi^\s(\Costhis|\Qhis)}{\Phi^{\sran}(\Costhis|\Qhis)}=  \sum_{\t=1}^{+\infty} \frac{\phibar^{\s}(\ct|\qt)}{\phibar^{\sran}(\ct|\qt)}=  \sum_{\k=1}^{+\infty} \frac{\phibar^{\s}(\ctk|\qtk)}{\phibar^{\sran}(\ctk|\qtk)}.
\end{align}


We further break the sequence $\(\qtk\)_{\k=1}^{\infty}$ into converging sub-sequences: Since $\(\qtk\)_{\k=1}^{\infty}$ is a bounded infinite sequence, we must be able to find a converging sub-sequence, denoted as $\hat{\Q}^1 \deleq \(\q^{\tk^1}\)_{\k=1}^{\infty}$, and the limit point is $\qhat^1$. If the remaining strategy profiles are finite, then we denote the remaining strategy profiles as $\hat{\Q}^0$. Otherwise, we can find the second converging sub-sequence, denoted as $\hat{\Q}^2 \deleq \(\q^{\tk^2}\)_{\k=1}^{\infty}$, and the limit point is $\qhat^2$. This process is continued iteratively

then we have a single converging (sub)-sequence ($m=1$), and we denote the limit point as $\qhat^1$. If $\(\qtk\)_{\k=1}^{\infty}$ is a divergent sequence, then can find a converging sub-sequence, denoted as 


We will show that $\thetabar(\s)=0$ for any such $\s$ with probability 1. 

From the definition of limit point, for any strategy profile $\qbar \in \limpq \cap \Qhats$, we can find a sub-sequence $\(\qtk\)_{\k =1}^{\infty}$ such that $\lim_{\k \to \infty} \qtk=\qbar$, and $D_{KL} \left(\phibar^{\sran}(\cbar|\qbar)||\phibar^{\s}(\cbar|\qbar)\right)>0$. We next show that 






Then from the definition of limit point, we know that for any $\q \in \limpq$, there exists a sub-sequence 
\QEDA

==> proof_convergence_eq.tex <==
%%novalidate

%%novalidate
% !TEX root = main041620.tex




% \vspace{0.2cm}

% \noindent\textbf{\emph{Proof of Proposition \ref{prop:map_stability}} .}
%  We prove the local stability property of learning with MAP estimator and equilibrium strategies. 

%  Firstly, we consider $\epsilonhat \deleq \frac{1}{|\S|}$. For any belief $\theta \in N_{\epsilonhat}\(\mathds{1}_{\thetabar_M}\)$, we can check that $\theta_M= \argmax_{\s \in \S}\theta=\thetabar_M$. Therefore, $\gwe(\theta_M)=\qbar$. Additionally, consider $\deltahat\deleq \min\{\loadepfin, \delta\}$. Then, for any $\q \in N_{\deltahat}\(\EQ(\thetabar_M)\) \subseteq N_{\delta}\(\EQ(\thetabar_M)\)$, $\thetabar_M \in \Sequiv(\q)$. Therefore, we have: 
% \begin{align*}
%     \lim_{\t \to \infty}\pro\(\thetat_M \in N_{\thetaepfin}\(\thetabar_M\), \qt \in N_{\loadepfin}\(\EQ(\thetabar_M)\)\) \geq   \pro\(\thetat_M=\thetabar_M, \qt \in N_{\deltahat}\(\EQ(\thetabar_M)\), ~\forall \t\)
% \end{align*}

% Secondly, we define: 
% \begin{align*}
%     \hat{\rho}^1= 
% \end{align*}
% Analogous to Lemma \ref{lemma:stopping_time}, we can show that if $0<\thetazero(\s)< \hat{\rho}^1$ for any $\s \in \S\setminus \{\thetabar_M\}$, then $\pro\(\thetat(\s)< \epsilonhat, ~ \forall \s \in \S \setminus \{\thetabar_M\}, ~ \forall \t\) > \gamma$. This implies that 

% Thirdly, analogous to Lemma \ref{lemma:other_parameters}

% Finally, analogous to the proof of Theorem \ref{theorem:stability_eq}, we can show that 

% The proof for learning with best response strategies is analogous to that for best response strategies, and hence is omitted. 
% \QEDA




% For each player $\i \in \I$ and any $\s \in [\thetabar]$, since $\s \in \Sequiv()$ we define a vector $\lambda_i \in \mathbb{R}^{dim\(\Qi\)}$ to be a feasible direction of perturbation if $\qi'=\qi + \xi \lambda_i$ is a feasible strategy of player $\i$ for sufficient small $\xi$. By choosing $\xi< \delta$, the perturbed strategy $\(\qi', \qmi\) \in N_{\delta}\(\EQ(\theta)\)$. Hence, from condition (ii), $[\thetabar] \in \Sequiv(\qi',\qmi)$. Therefore, we must have $u_i^s(\qi', \qmi)$ for all $\s \in [\thetabar]$. Since the utility function $u_i^s(\q)$ is differentiable in $\q$, we can calculate the directional derivative as follows: 
% \begin{align*}
% \nabla_{\lambda_i} \usi(\qi, \qmi) =&\lim_{\xi \to 0} \frac{\usi(\q_i+ \xi \lambda_i, \qmi)-\usi(\qi, \qmi)}{\xi}\\
% =&\lim_{\xi \to 0} \frac{u_i^{\sran}(\q_i+ \xi \lambda_i, \qmi)-u_i^{\sran}(\qi, \qmi)}{\xi} =  \nabla_{\lambda_i} u_i^{\sran}(\qi, \qmi), \quad \forall \s \in [\thetabar].
% \end{align*}

% % Since the payoff equivalent parameter set $\Sequiv(\qbar)$ is identical for all $\qbar \in \EQ(\thetabar)$, we denote $\Sequiv \deleq \Sequiv(\qbar)$ for any $\qbar \in \EQ(\thetabar)$. We now show that for any $\s \in \Sequiv$ and any $\q \in \EQ(\theta)$, $\nabla_{\lambda_i} \usi(\qi, \qmi) = \nabla_{\lambda_i} u_i^{\sran}(\qi, \qmi)$ for any feasible perturbation direction $\lambda_i$ of each player $\i$'s strategy. Note that for any $\s \in \Sequiv$, $\usi(\q')=u_i^{\sran}(\q')$ for any $\q' \in N_{\delta}(\q)$. Therefore, for any $\i \in \I$, any feasible direction $\lambda_i$, any $\s \in \Sequiv$, and any $\q \in \EQ(\theta)$ we have: 

% Then, 
% \begin{align}\label{eq:expected_derivative}
% \nabla_{\lambda_i} \mathbb{E}_{\thetabar}[u_i^{\s}(\qi, \qmi)]= \sum_{\s \in \S} \thetabar(\s) \nabla_{\lambda_i} \usi(\qi, \qmi) = \nabla_{\lambda_i} u_i^{\sran}(\qi, \qmi).
% \end{align}
% Since $\qi$ is a best response strategy of $\qmi$ given $\thetabar$, $\qi$ must be a local maximizer of the expected utility function $\mathbb{E}_{\thetabar}[u_i^{\s}(\qi, \qmi)]$. From \eqref{eq:expected_derivative}, $\qi$ is also a local maximizer of the utility function with the true parameter $u_i^{\sran}(\qi, \qmi)$. Since the utility function $\usi(\qi, \qmi)$ is concave in $\qi$ for all $\s \in [\thetabar]$, $\qi$ is a global maximizer of $\mathbb{E}_{\thetabar}[u_i^{\s}(\qi, \qmi)]$ and $u_i^{\sran}(\qi, \qmi)$. Therefore, $\qi$ is a best response strategy with respect to $\qmi$ with complete information of $\sran$. We can thus conclude that $\q$ must be a complete information equilibrium. 
% \QEDA 


%\noindent\textbf{\emph{Proof of Lemma \ref{lemma:constrained_set}.}} For any $\loadepfin$, we define $\deltahat \deleq \min\{\loadepfin, \delta\}$ and $\neighhatload \deleq N_{\deltahat}\(\EQ(\thetabar)\)$. From the sufficient condition, we know that for any $\q \in \neighhatload$, $\Sequiv(\q)=\Sstar$. Since $\EQ(\theta)$ is upper-hemicontinuous in $\theta$, we can find a positive number $\epsilon'$ such that for any $\theta \in N_{\epsilon'}(\thetabar)$, $\EQ(\theta) \subseteq \neighhatload$. Then, for any $\thetaepfin$, we take $ \epsilonhat = \min\left\{\frac{\epsilon'}{|\S|}, \frac{\thetaepfin}{|\S|}\right\}$ and define $\neighhattheta\deleq \left\{\theta\left \vert \theta(\s)-\thetabar(\s)<\epsilonhat, ~\forall ~ \s \in \S\right.\right\}$. For any $\theta \in \neighhattheta$, we have $\|\theta-\thetabar\|< \epsilon'$ so that $\EQ(\theta) \subseteq\neighhatload$ and hence $\Sequiv(\q)=\Sstar$ for all $\q \in \EQ(\theta)$. Since $\epsilonhat \leq \frac{\thetaepfin}{|\S|}$ and $\deltahat \leq \loadepfin$, we know that $\Thetahat \in N_{\thetaepfin}(\thetabar)$ and $\Qhat \subseteq N_{\loadepfin}(\EQ(\thetabar))$. Therefore, $\pro\(\thetat \in \Thetahat, ~ \qt \in \Qhat, ~ \forall \t\)\leq \pro\(\thetat \in N_{\thetaepfin}(\thetabar), ~ \qt \in N_{\loadepfin}(\EQ(\thetabar)), ~ \forall \t\)$. \QEDA 


    
    
      
%    \vspace{0.2cm}
%
%\noindent\textbf{\emph{Proof of Corollary \ref{cor:identified}.}} From Theorem \ref{theorem:convergence_eq}, we know that the belief $\thetabar$ must exclude all parameters that are not payoff equivalent, and hence must exclude all $\s \in \S \setminus \{\sran\}$. Therefore, $\thetabar=\thetasran$ and $\qbar \in \EQ(\thetasran)$ with probability 1. 
%\QEDA












==> review_sa.tex <==
%%novalidate
% \section{Review of Asynchronous Stochastic Approximation Theory}\label{apx:asynchronous}

% For any belief $\theta \in \Delta(\S)$, we consider the following iterative process of $\(\qt\)_{\t=1}^{\infty}$: 
% \begin{align}\label{eq:residual}
%     \qi^{\t+1}&=(1-\ait)\qit+ \ait \gibr(\theta, \qt) + \xi_i^{\t+1}, \quad \forall \i \in \I, \quad \forall \t,
% \end{align}
% where $\gibr(\theta, \qt) \in \BRi(\theta, \qt)$ is a best-response strategy of player $\i$ based on the belief $\theta$ and the current strategy profile $\qt$. For each $\t$, $\xi_i^{\t} \in \mathbb{\R}^{dim(\Q)}$. If $\xi^\t=0$ for all $\t$, then the dynamics in \eqref{eq:residual} is the asynchronous best-response dynamics with a fixed belief $\thetat=\theta$ as in \eqref{eq:br_update}.  We make the following assumption on the sequence $\(\xi^\t\)_{\t=1}^{\infty}$:

% \textbf{(A7)} For any $\t$, $\xi^{\t}$ is bounded. Additionally, $\lim_{\t \to \infty} \xi^\t=0$.

% For any strategy sequence $\(\qt\)_{\t=1}^{\infty}$, we consider the following linear interpolation function $x(\tau): [0, \infty) \to \Q$ of $\(\qt\)_{\t=1}^{\infty}$: \begin{align}\label{eq:interpolate}
%     x\(\hat{\tau}_{\t}+ t\) =\qt+ t \frac{\q^{\t+1}-\qt}{\abar^{\t}}, \quad \forall t\in [0, \abar^{\t}), \quad \forall \t=1, 2, \dots,
% \end{align}
% where $\abar^j=\max_{\i \in \I} a_i^{j}$, $\hat{\tau}_1=0$, and $\hat{\tau}_{\t}=\sum_{j=1}^{\t-1} \abar^{j}$ for all $\t=2, 3,\dots$.


% We also consider the following differential inclusion: 




% \begin{definition}[\cite{benaim2005stochastic}]\label{def:flow}
% We define the flow induced by the differential inclusion \eqref{eq:differential_inclusion} with initial strategy $\q$ as $\Phi_\t(q) = \left\{\tilde{q}(\tau): \tilde{q}(\tau) \text{ is a solution to \eqref{eq:differential_inclusion} with $\tilde{\q}(0)=q$.}\right\}$
% \end{definition}
% \begin{definition}[\cite{benaim2005stochastic}]\label{def:pesudo}
% A continuous function $x: [0, \infty) \to \Q$ 
% is an asymptotic pseudo-trajectory to $\Phi$ if for any $K>0$,
% \begin{align*}
%     \lim_{\tau\to \infty} \sup_{t \in [0, K]} d\(x(t+\tau), \Phi_{t}\(\tilde{\q}(\tau)\)\)=0.
% \end{align*}
% \end{definition}

% \begin{lemma}[\cite{perkins2013asynchronous}]\label{lemma:approximate}
%   Under the assumptions \textbf{(A3)} -- \textbf{(A5)} and \textbf{(A7)}, for any belief $\theta \in \Delta(\S)$, the interpolation function
% $x(\tau)$ given by \eqref{eq:interpolate} is an asymptotic pseudo-trajectory to the differential inclusion \eqref{eq:differential_inclusion} with probability 1.
% \end{lemma}




% \begin{lemma}[\cite{perkins2013asynchronous}]\label{lemma:asynchronous}
%  Under Assumptions \textbf{(A3)} -- \textbf{(A6)} and \textbf{(A7)}, for any belief $\theta$, the sequence $\(\qt\)_{\t=1}^{\infty}$ given by \eqref{eq:residual} converges to the equilibrium set $\EQ(\theta)$ with probability 1. 
% \end{lemma}


